Ranking and synchronization from pairwise measurements via SVD

Given a measurement graph $G= (V,E)$ and an unknown signal $r \in \mathbb{R}^n$, we investigate algorithms for recovering $r$ from pairwise measurements of the form $r_i - r_j$; $\{i,j\} \in E$. This problem arises in a variety of applications, such as ranking teams in sports data and time synchronization of distributed networks. Framed in the context of ranking, the task is to recover the ranking of $n$ teams (induced by $r$) given a small subset of noisy pairwise rank offsets. We propose a simple SVD-based algorithmic pipeline for both the problem of time synchronization and ranking. We provide a detailed theoretical analysis in terms of robustness against both sampling sparsity and noise perturbations with outliers, using results from matrix perturbation and random matrix theory. Our theoretical findings are complemented by a detailed set of numerical experiments on both synthetic and real data, showcasing the competitiveness of our proposed algorithms with other state-of-the-art methods.

==> AAA_todo.tex <==
table of contents in red?
check acknowledgements 

Shall we say in Remark 4, paragraph 1, that 

we run into computational issues when running matrix completion for n>3000 and even sparse graphs p=5\%? Just to make it clear how slow this method actually is... 




==> prelim_exp.tex <==



%\vspace{-2mm}
\paragraph{NCAA College Basketball.} Our final real data set comes from sports, and contains the outcomes of NCAA College Basketball matches during the regular season, for the years $1985$ - $2014$. The left plot of Figure \ref{fig:NBA}  shows the number of upsets across time, while the right plot shows the average over the entire period, for each algorithm. 
On average, it is typically the case that a pair of teams play each other at most once. We remark that the number of upsets shown in Figure \ref{fig:NBA} (left) is ascending since the number of teams grew over the years. 
% 
For example, during the $1985$ season, the league contained $282$ teams and $3737$ games took place, while in $2014$, there were $351$ teams and $5362$ games.
%%% , with each team playing on average about 30 games.
We remark that, on average, the best performer was \textsc{RC} followed by \textsc{SVDN}, and that  \textsc{GLM} was by far the worst performer. 

%\vspace{-1mm}
\begin{figure}[!ht]
\centering
\subcaptionbox[]{ Yearly number of upsets.
% \label{subfig:sublabel3}
}[ 0.24\columnwidth ]
{\includegraphics[width=0.24\columnwidth] {PLOTS2019/realData/Basketball_nrUpsets_byYear_1.png} }
% \hspace{0.01\columnwidth} % seperation
%
\subcaptionbox[]{ Average over 1984 - 2014 % number of upsets.
% \label{subfig:sublabel3}
}[ 0.24\columnwidth ]
{\includegraphics[width=0.24\columnwidth] {PLOTS2019/realData/Basketball_nrUpsets_byYear_Averaged_1.png} }
% \hspace{0.01\columnwidth} % seperation
%\vspace{-1mm}
\captionsetup{width=0.98\linewidth}
\caption[Short Caption]{Number of upsets in basketball data. %  1984 - 2014.
% Comparison of algorithms for the basketball data set 1984 - 2014.
}
\label{fig:NBA}
\end{figure}
%\vspace{-1mm}







\end{document}



==> svdRank_ERO_proof_ell2_thm.tex <==
%-----------------------------------------
% Proof of Theorem \ref{eq:main_thm_ERO}
%-----------------------------------------

\section{Proof of Theorem \ref{thm:main_thm_ERO}}  \label{sec:proofThm_ERO}
%
%--------------------------------------------------------------------------
% Step 1: Analysis of the singular values and singular vectors of $C$
%--------------------------------------------------------------------------
\subsection{Step 1: Analysis of the singular values and singular vectors of $C$} \label{subsec:step1_ero_proof}
%
%---------
% Proof
%---------
\begin{proof}[Proof of Lemma \ref{lem:sing_vals_C}]
We begin by noting that for $\alpha = \frac{r^T e}{n}$, $\dotprod{e}{r-\alpha e} = 0$ and so $u_1, u_2$ (similarly $v_1,v_2$) 
are orthogonal. Moreover, $u_1,u_2,v_1,v_2$ also have unit $\ell_2$ norm. Finally, we note that 
%
\begin{equation*}
u_1 v_1^T + u_2 v_2^T 
= \frac{1}{\sqrt{n}\norm{r-\alpha e}_2}[-e(r-\alpha e)^T + (r-\alpha e) e^T] 
= \frac{1}{\sqrt{n}\norm{r-\alpha e}_2}[\underbrace{r e^T - e r^T}_{C}], 
\end{equation*}
%  
which completes the proof.	
\end{proof}

%------------------------------------------
% Step 2: Bounding the spectral norm of Z
%------------------------------------------
\subsection{Step 2: Bounding the spectral norm of Z} \label{subsec:step2_ero_proof}

%
%
\begin{proof}[Proof of Lemma \ref{lem:specnorm_Z_ERO}]
We begin by considering the second moment of $S_{ij}$ for $i < j$. Note that $\expec[N_{ij}] = 0$ and 
$\expec[N_{ij}^2] = M^2/3$. We thus obtain
%
\begin{align*}
\expec[ (S)_{ij}^2 ]   
& =  
\eta p (1- \eta p)^2 (r_i - r_j)^2  
+ (1-\eta) p  \expec[ N_{ij} - \eta p (r_i - r_j) ]^2 
+ (1- p) (r_i - r_j)^2 \eta^2 p^2  \\
& =
\eta p (1- \eta p)^2 (r_i - r_j)^2  
+ (1-\eta) p  \left[  \frac{M^2}{3}  + \eta^2 p^2 (r_i - r_j)^2 \right]  + (1- p) (r_i - r_j)^2 \eta^2 p^2 
\end{align*}
%
%
which together with $ (r_i - r_j)^2  \leq M^2$ yields 
%
\begin{align*}
\expec[ (S)_{ij}^2 ]
& \leq  \eta p (1- \eta p)^2 M^2 + (1-\eta) p \left[ \frac{M^2}{3} + \eta^2 p^2 M^2 \right] + (1- p) \eta^2 p^2 M^2  \\
& = [ \eta p (1-\eta p )^2 + (1-\eta) p \left(\frac{1}{3}+\eta^2p^2 \right) + (1-p) \eta^2 p^2  ] M^2 \\
&\leq \left(\eta p + \frac{4}{3}p + \eta^2 p^2 \leq \frac{10}{3}p \right) M^2 = \frac{10p}{3} M^2.
\end{align*}
%
We thus have that $ \expec[ (S)_{ij}^2 ] \leq  \frac{10p}{3} M^2$ for $i < j$; the same bound holds for $i > j$ as well. 
Hence we can bound the quantities $\tilde{\sigma}, \tilde{ \sigma }_*$ defined in Theorem \ref{app:thm_symm_rand} as 
follows.
%
\begin{align*}
\tilde{\sigma} & :=  \max_{i}  \sqrt{ \sum_{j}   \expec[ (\tilde{S})_{ij}^2 ]  }  
 \leq  \sqrt{ \frac{10p}{3} n  M^2 } = M \sqrt{\frac{10p}{3} n } , \\
%
   \tilde{ \sigma }_* &:=  \max_{i,j} ||  (\tilde{S})_{ij}   ||_{\infty}  \leq 2M. 
   %(n-1) (1+ \eta p)  \leq n (1+\eta p) .
\end{align*}
%
%
Then by invoking Theorem \ref{app:thm_symm_rand}, we obtain for any given $t \geq 0$, $0 < \varepsilon \leq 1/2$ that
%
\begin{align*}
\mathbb{P}( || \tilde{S} ||_2  \geq (1+\varepsilon) 2 \sqrt{2}  M \sqrt{\frac{10p}{3} n}  + t)
&\leq \mathbb{P}( || \tilde{S} ||_2  \geq (1+\varepsilon) 2 \sqrt{2}  \tilde{\sigma}  + t)    \\
& \leq 2n \exp  \left( \frac{-t^2}{c_{\varepsilon} \sigma_*^2 } \right) 
\leq 2n \exp  \left( \frac{-t^2}{4 c_{\varepsilon} M^2  } \right),  
\end{align*}
%
where $c_{\varepsilon} > 0$ depends only on $\varepsilon$. 
Plugging   $t = 2 \sqrt{2} M \sqrt{\frac{10p}{3} n}$ we obtain the stated bound. 
%
\end{proof}
%
%------------------------------
% Step 3: Using Wedin's bound
%------------------------------ 
\subsection{Step 3: Wedin's bound} \label{subsec:step3_ero_proof}
%
%
%
\begin{proof}[Proof of Lemma \ref{lem:wedins_bd_ero}]
Note that Weyl's inequality \cite{Weyl1912} (see Theorem \ref{thm:weyl_sing_values}) 
for singular value perturbation readily yields 
%
\begin{equation*}
   \sigma_i(H) \in [ \sigma_i( \eta p C )  \pm \Delta ], \quad \forall  i =1,\ldots,n.
\end{equation*}
%
In particular, using the expressions for $\sigma_1(C), \sigma_2(C)$ from Lemma \ref{lem:sing_vals_C}, 
we have that 
%
\begin{align*}
   \sigma_1(H), \sigma_2(H)  &\geq  \eta p  \sqrt{n} \norm{r-\alpha e}_2 - \Delta, \\ 
	\sigma_3(H),  \ldots,  \sigma_n(H)  &\leq  \Delta.
\end{align*}
%
% 
%Let us denote $U = [u_1 \ u_2] \in \matR^{n \times 2}$ where we recall from Lemma \ref{lem:sing_vals_C} 
%that $ u_1 = \frac{e}{\sqrt{n}},  u_2 = - \frac{(r-\alpha e)}{ || r-\alpha e ||_2 }  $ are the left singular 
%vectors corresponding to the non-zero singular values of $C$. Also, let us denote 
%$\hat U = [\hat u_1 \ \hat u_2] \in \matR^{n \times 2}$ where $\hat u_1 , \hat u_2$ are the left singular vectors
%corresponding to the top two singular values of $H$.
Then using Wedin's bound for perturbation of singular subspaces \cite{Wedin1972} (see Theorem \ref{thm:wedin_bd}), 
we obtain
%
\begin{equation*} %\label{eq:sintheta_bd_1}
||  \sin \Theta(\calR(\hat{U}), \calR(U))  ||_2 = ||  (I - \hat{U} \hat{U}^T) U  ||_2  
 \leq  \frac{ \Delta }{  \eta p  \sqrt{n} \norm{r-\alpha e}_2 - \Delta }  \ (=: \delta) 
\end{equation*}
%
%
provided $\Delta <  \eta p  \sqrt{n} \norm{r-\alpha e}_2$ holds. 
\end{proof}

%--------------------------------
% Analyzing the projection step
%--------------------------------
\subsection{Step 4: Analyzing the projection step} \label{subsec:step4_ero_proof}
%
%
\begin{proof}[Proof of Lemma \ref{lem:proj_analysis_Step_ERO}]
To begin with, note that $ \bar{u}_1 = \hat{U} \hat{U}^T u_1$  is the orthogonal projection 
of $u_1$ on $\calR(\hat{U})$. A unit vector orthogonal to $ \bar{u}_1 $ and lying in $\calR(\hat{U})$ is given by 
%
%
\begin{equation*}
	\tilde{u}_2 = \frac{1}{ || \bar{u}_1 ||_2 } \;  \hat{U}     \; 
\begin{bmatrix}
  \mp  \langle \hat{u}_2, \bar{u}_1  \rangle    \\
  \pm    \langle \hat{u}_1, \bar{u}_1  \rangle
\end{bmatrix} .
\end{equation*}
%
% 
%
Denoting $ \bar{u}_2$ to be the orthogonal projection of $u_2$ on $ \calR(\hat{U})$,  we can decompose 
$\langle \tilde{u}_2, u_2  \rangle$ as
%
\begin{equation*}
 \langle \tilde{u}_2, u_2  \rangle =   \langle \tilde{u}_2,   
u_2 - \frac{ \bar{u}_2 }{|| \bar{u}_2 ||_2 } \rangle +   \langle \tilde{u}_2, 
\frac{ \bar{u}_2 }{|| \bar{u}_2 ||_2 } \rangle,
\end{equation*}
%
which leads to 
%
\begin{equation} \label{eq:lowbd_u2til_u2}
|  \langle \tilde{u}_2, u_2  \rangle  |     
\geq  
 		| \langle \tilde{u}_2,   \frac{ \bar{u}_2 }{|| \bar{u}_2 ||_2 } \rangle |
     -  |  \langle \tilde{u}_2,   u_2 - \frac{ \bar{u}_2 }{|| \bar{u}_2 ||_2 } \rangle  | .
\end{equation}
%
%
We will now bound the two terms in the RHS of \eqref{eq:lowbd_u2til_u2} starting with the first term.

%--------------------------
% Bounding the first term
%--------------------------
\underline{\textbf{Lower bounding the first term in RHS of \eqref{eq:lowbd_u2til_u2}.}} 
Since $\dotprod{\hat u_2}{\bar{u}_1} = \dotprod{\hat u_2}{u_1}$,  $\dotprod{\hat u_1}{\bar{u}_1} = \dotprod{\hat u_1}{u_1}$, we obtain
%
%
\begin{align*}
 \langle \tilde{u}_2,   \frac{ \bar{u}_2 }{|| \bar{u}_2 ||_2 } \rangle
& = \frac{u_2^T}{ || \bar{u}_1||_2  ||  \bar{u}_2 ||_2 }  \hat{U}       \underbrace{ \hat{U}^T    \hat{U}  }_{I}
\begin{bmatrix}
  \mp  \langle \hat{u}_2, \bar{u}_1  \rangle    \\
  \pm    \langle \hat{u}_1, \bar{u}_1  \rangle
\end{bmatrix}   \\
%
& = \frac{1}{\norm{\bar{u}_1}_2 \norm{\bar{u}_2}}_2 
[\mp\dotprod{u_2}{\hat u_1} \dotprod{\hat u_2}{u_1} \pm \dotprod{u_2}{\hat u_2}\dotprod{\hat u_1}{u_1}] \\
& = \frac{1}{\norm{\bar{u}_1}_2 \norm{\bar{u}_2}}_2 [\pm \det(U^T \hat U)]. \label{eq:lowbd}
\end{align*}
%
%
Recall the definition of $\delta$ in \eqref{eq:sintheta_bd_1}. The following simple claims will be useful for us. 
%
\begin{claim} \label{claim:detbd}
With $\delta$ as defined in \eqref{eq:sintheta_bd_1} we have $\abs{\det(U^T \hat U)} \geq 1 - \delta^2$.
\end{claim}
%
\begin{proof}
Since $U^T \hat U$ is a $2 \times 2$ matrix, we have that
%
\begin{equation*}
\abs{\det(U^T \hat U)} \geq \sigma_{min}^2(U^T \hat U) = 1 - ||  \sin \Theta(\calR(\hat{U}), \calR(U))  ||_2^2 \geq 1-\delta^2.
\end{equation*}
%
\end{proof}
%
\begin{claim} \label{claim:u1u2_proj_err}
It holds that $\norm{\bar{u}_1 - u_1}_2, \norm{\bar{u}_2 - u_2}_2 \leq \delta$.
\end{claim}
%
\begin{proof}
We will only show the bound for $\norm{\bar{u}_1 - u_1}_2$ as an identical argument holds for 
bounding $\norm{\bar{u}_2 - u_2}_2$. Using the facts $\bar u_1 = \hat U \hat U u_1$ and 
$u_1 = U U^T u_1$, we obtain
%
\begin{align*}
\norm{u_1 - \bar{u}_1}_2 
= \norm{(I -  \hat U \hat U^T)u_1}_2 = \norm{(I -  \hat U \hat U^T)U U^T u_1}_2 
\leq \norm{(I -  \hat U \hat U^T)U U^T}_2 = \norm{(I -  \hat U \hat U^T)U}_2 \leq \delta
\end{align*}
%
where the last inequality follows from \eqref{eq:sintheta_bd_1}.
\end{proof}
%
%
Using Claims \ref{claim:detbd}, \ref{claim:u1u2_proj_err} we can lower bound the 
first term in RHS of \eqref{eq:lowbd_u2til_u2} as follows.
%
\begin{equation}
\abs{ \langle \tilde{u}_2,   \frac{ \bar{u}_2 }{|| \bar{u}_2 ||_2 } \rangle }  
\geq \frac{1 - \delta^2}{(1+\delta)^2} = \frac{1-\delta}{1+\delta} = 1 - \frac{2 \delta}{1+\delta} \geq 1-2 \delta.
\label{eq:FirstTermFinalBound}
\end{equation}
%

%-----------------------------------
% Upper bounding the second term
%----------------------------------- 
\underline{\textbf{Upper bounding the second term in RHS of \eqref{eq:lowbd_u2til_u2}.}}
%
We can do this as follows.
%
\begin{align}
\abs {\langle \tilde{u}_2, u_2 - \frac{ \bar{u}_2  }{  || \bar{u}_2 ||_2 } \rangle }  
&\leq  \norm{   u_2 - \frac{ \bar{u}_2  }{  || \bar{u}_2 ||_2 }   }_2 \quad 
(\text{Cauchy-Schwartz and since } \norm{\tilde{u}_2}_2 = 1) \nonumber  \\
%%
&  = \norm{  u_2 - \bar{u}_2 + \bar{u}_2 - \frac{ \bar{u}_2 }{ ||  \bar{u}_2 ||_2 } }_2  \nonumber \\ 
%
&\leq \norm{u_2 - \bar{u}_2}_2 + \norm{\bar{u}_2 - \frac{ \bar{u}_2 }{ ||  \bar{u}_2 ||_2}}_2 \nonumber  \\
%
&\leq  \delta + \abs{ 1 - \frac{ 1 }{ || \bar{u}_2 ||_2 }  }  \quad (\text{ Using Claim \ref{claim:u1u2_proj_err}}) \nonumber  \\
&= \delta + \frac{ \abs{ || \bar{u}_2 ||_2 - 1 } }{ || \bar{u}_2 ||_2 } \nonumber  \\
&  \leq \delta + \frac{\delta}{1-\delta}  \quad 
(\text{since } || \bar{u}_2 ||_2 \in [1-\delta,1+\delta]  \text{ from Claim \ref{claim:u1u2_proj_err}}) \nonumber \\
%
&\leq 3 \delta  \quad  (\mbox{whenever } \; \delta \leq 1/2).  \label{eq:SecTermFinalBound}
\end{align}
% 
Altogether, we conclude that if $\delta \leq 1/2$ then using \eqref{eq:FirstTermFinalBound}, 
\eqref{eq:SecTermFinalBound} in \eqref{eq:lowbd_u2til_u2}, we obtain
%
%
\begin{equation*}
| \langle \tilde{u}_2,  u_2 \rangle | \geq  1 - 5 \delta,  
\end{equation*}
%
%
and consequently, there exists $ \beta \in \{ -1, 1 \}$ such that  
%
\begin{equation} \label{eq:l2normbd_1}
|| \tilde{u}_2 - \beta  u_2  ||_2^2 = 2 - 2 \langle \tilde{u}_2,  \beta u_2 \rangle  \leq 10 \delta.
\end{equation}
\end{proof}
%
%
%--------------------------------
% Step 5: Putting it together
%--------------------------------
\subsection{Step 5: Putting it together} \label{subsec:step5_ero_proof}
From the definition of $\delta$ in \eqref{eq:sintheta_bd_1}, we can easily see that  
%
\begin{equation}
\delta \leq 1/2 \Leftrightarrow 3 \Delta  \leq   \eta p  \sqrt{n} \norm{r-\alpha e}_2  .
\label{eq:3delta}
%
\end{equation}
%
Plugging $\Delta = 4 \sqrt{2}  \sqrt{\frac{10p}{3} n} M  (2 + \varepsilon) $ from 
\eqref{eq:Delta_bd} in \eqref{eq:3delta}, we then arrive at 
%
%
\begin{align}
12 \sqrt{2}  \sqrt{\frac{10p}{3} n} M (2+\varepsilon)  &\leq  \eta p \norm{r-\alpha e}_2 \sqrt{n} \nonumber \\
%
\Leftrightarrow \norm{r-\alpha e}_2 &\geq  \frac{24 M}{\eta}  \sqrt{\frac{5}{3p}} (2 + \varepsilon). 
\label{eq:tempbd}
\end{align}
%
%
Finally, if $\Delta$ satisfies the bound in \eqref{eq:3delta}, we obtain, starting 
from the definition of $\delta$, that
% 
%
\begin{align*}
\delta &:= \frac{ \Delta }{  \eta p  \norm{r-\alpha e}_2 \sqrt{n} - \Delta } \\
%
&\leq \frac{ 3 \Delta }{ 2 \eta p  \norm{r-\alpha e}_2 \sqrt{n} } 
\quad (\text{using \eqref{eq:3delta}}) \\
%
&= \frac{12 M}{\eta} \sqrt{\frac{5}{3p}} \frac{(2+\varepsilon)}{\norm{r-\alpha e}_2}
\quad (\text{using expression for $\Delta$ from \eqref{eq:Delta_bd}}) .
\end{align*}
%
%
Plugging this in \eqref{eq:l2normbd_1} yields the stated bound on $||  \tilde{u}_2 - \beta u_2 ||_2^2 $.

==> svdRank_ERO_proof_ellinf_thm.tex <==
%--------------------------------------------------------------
% Proof of Lemmas from Section \ref{thm:main_thm_linfty_ERO}
%--------------------------------------------------------------
\section{Proof of Lemmas from Section \ref{thm:main_thm_linfty_ERO}}
%
%
\subsection{Proof of Lemma \ref{linf_ero_step1}} 
%
\begin{proof}
Recall from the proof of Lemma \ref{lem:proj_analysis_Step_ERO} that 
%
\begin{equation} \label{eq:linf_step1_temp1}
	\tilde{u}_2 = \frac{1}{ || \bar{u}_1 ||_2 } \;  \hat{U}     \; 
\begin{bmatrix}
  \mp  \langle \hat{u}_2, \bar{u}_1  \rangle    \\
  \pm    \langle \hat{u}_1, \bar{u}_1  \rangle
\end{bmatrix} 
%
= \frac{1}{ || \bar{u}_1 ||_2 } \;  \hat{U}     \; 
\begin{bmatrix}
  0 & \mp1 \\
	\pm1 & 0
\end{bmatrix} \Uhat^T \bar{u}_1 
%
= \frac{1}{ || \bar{u}_1 ||_2 } \;  \hat{U}     \; 
\begin{bmatrix}
  0 & \mp1 \\
	\pm1 & 0
\end{bmatrix} \Uhat^T u_1, 
\end{equation}
%
%
where the last equality follows from the fact 
$\dotprod{\hat u_2}{\bar{u}_1} = \dotprod{\hat u_2}{u_1}$,  $\dotprod{\hat u_1}{\bar{u}_1} = \dotprod{\hat u_1}{u_1}$.
Let $O$ be any $2 \times 2$ orthogonal matrix, clearly, $UO$ also corresponds to the two largest left singular vectors 
of $\expec[H]$ (since $\sigma_1(\expec[H]) = \sigma_2(\expec[H])$). Denote $P = \Uhat - U$. Plugging in \eqref{eq:linf_step1_temp1}, we obtain 
%
% 
\begin{align}
	\tilde{u}_2 &= \frac{1}{ || \bar{u}_1 ||_2 } \;  \hat{U}     \; 
\underbrace{\begin{bmatrix}
  0 & \mp1 \\
	\pm1 & 0
\end{bmatrix}}_{D} \Uhat^T \bar{u}_1  [O^T U^T + P] u_1 \nonumber \\
%
%
&= \pm \det(O) u_2 + \underbrace{\frac{1}{ || \bar{u}_1 ||_2 } UO D P^T u_1}_{w_1} + \underbrace{\frac{1}{ || \bar{u}_1 ||_2 } PDO^T U^T u_1}_{w_2} 
+ \underbrace{\frac{1}{ || \bar{u}_1 ||_2 } PDP^T u_1}_{w_3} \nonumber \\
%
\Rightarrow \norm{\tilde{u}_2 \mp \det(O) u_2}_{\infty} &\leq \norm{w_1}_{\infty} + \norm{w_2}_{\infty} + \norm{w_3}_{\infty}. \label{eq:u2til_inf_bd_init}
\end{align}
%
Denoting 
%
\begin{equation*}
P = [p_1 \ p_2], \quad O = \begin{bmatrix}
  o_{11} & o_{12} \\
	o_{21} & o_{22}
\end{bmatrix}
\end{equation*}
%
we will now bound $\norm{w_1}_{\infty} , \norm{w_2}_{\infty} , \norm{w_3}_{\infty}$. 

%------ Bounding w_1 infty norm --------
To begin with, 
%
\begin{align}
w_1 &= \frac{1}{\norm{\bar{u}_1}_2} [u_1 \ u_2] O 
\begin{bmatrix}
  0 & \mp1 \\
	\pm1 & 0
\end{bmatrix} 
\begin{bmatrix}
  \dotprod{p_1}{u_1} \\
	\dotprod{p_2}{u_1}
\end{bmatrix} \nonumber \\
%
%
&= \frac{1}{\norm{\bar{u}_1}_2} [u_1 \ u_2] O 
\begin{bmatrix}
  \mp \dotprod{p_2}{u_1} \\
	\pm \dotprod{p_1}{u_1}
\end{bmatrix} \nonumber \\ 
%
%
&= \frac{1}{\norm{\bar{u}_1}_2} 
\begin{bmatrix}
  \mp o_{11}\dotprod{p_2}{u_1} \pm o_{12} \dotprod{p_1}{u_1} \\
	\mp o_{21}\dotprod{p_2}{u_1} \pm o_{22} \dotprod{p_1}{u_1}
\end{bmatrix} \nonumber \\
%
\Rightarrow \norm{w_1}_{\infty} &\leq 
\frac{1}{\norm{\bar{u}_1}_2} \left[(\abs{\dotprod{p_2}{u_1}} + \abs{\dotprod{p_1}{u_1}})(\norm{u_1}_{\infty} + \norm{u_2}_{\infty}) \right]. \label{eq:linf_step1_temp2}
\end{align} 
%
Clearly, $\norm{u_1}_{\infty} = \frac{1}{\sqrt{n}}$ and $\norm{u_2}_{\infty} \leq \frac{M - \alpha}{\norm{r - \alpha e}_2}$. 
Using H\"older's inequality,
% 
\begin{equation*}
	\abs{\dotprod{p_i}{u_1}} \leq \norm{P}_{\max} \norm{u}_1 = \norm{P}_{\max}\sqrt{n}; \quad i=1,2.
\end{equation*}
%
Moreover, from Claim \ref{claim:u1u2_proj_err}, we know that $\norm{\bar{u}_1}_2 \geq 1 - \delta$ where we recall $\delta$ defined in \eqref{eq:sintheta_bd_1}. 
We saw in \eqref{eq:3delta} that $\Delta \leq \frac{\eta p ||r-\alpha e||_2 \sqrt{n}}{3} \Leftrightarrow \delta \leq 1/2$, which implies 
$\norm{\bar{u}_1}_{2} \geq 1/2$. Plugging these bounds in \eqref{eq:linf_step1_temp2}, we obtain
%
\begin{equation} \label{eq:linf_w1_bd}
  \norm{w_1}_{\infty} \leq 4\norm{P}_{\max}\left(1 + \frac{\sqrt{n}(M-\alpha)}{\norm{r-\alpha e}_2} \right).
\end{equation}
%

%---------- Bounding w_2 infty norm --------
Next, we can bound $\norm{w_2}_{\infty}$ as follows.
\begin{align}
w_2 &= \frac{1}{\norm{\bar{u}_1}_2} [p_1 \ p_2] 
\begin{bmatrix}
  0 & \mp1 \\
	\pm1 & 0
\end{bmatrix} 
O^T
\begin{bmatrix}
  1 \\
	0
\end{bmatrix} \nonumber \\
%
&= \frac{1}{\norm{\bar{u}_1}_2} [p_1 \ p_2]
%
\begin{bmatrix}
  \mp o_{12} \\
	\pm o_{11}
\end{bmatrix} \nonumber \\ 
%
%
\Rightarrow \norm{w_2}_{\infty} &\leq \frac{2\norm{P}_{\max}}{\norm{\bar{u}_1}_2} \leq 4\norm{P}_{\max} \label{eq:w2_infty_bd}
\end{align}
%
since $\Delta \leq \frac{\eta p ||r-\alpha e||_2 \sqrt{n}}{3}$. 

%---------- Bounding w_3 infty norm --------
We now bound $\norm{w_3}_{\infty}$. 
%
\begin{align}
 w_3 &= \frac{1}{\norm{\bar{u}_1}_2} [p_1 \ p_2] 
\begin{bmatrix}
  0 & \mp1 \\
	\pm1 & 0
\end{bmatrix} 
\begin{bmatrix}
  \dotprod{p_1}{u_1} \\
	\dotprod{p_2}{u_1}
\end{bmatrix} \nonumber \\ 
&= 
%
\frac{1}{\norm{\bar{u}_1}_2} [p_1 \ p_2] 
\begin{bmatrix}
  \mp \dotprod{p_2}{u_1} \\
	\pm \dotprod{p_1}{u_1}
\end{bmatrix} \nonumber \\
%
\Rightarrow \norm{w_3}_{\infty} 
&\leq \frac{1}{\norm{\bar{u}_1}_2} ((\abs{\dotprod{p_2}{u_1}} + \abs{\dotprod{p_1}{u_1}}) \norm{P}_{\max})  \nonumber \\
&\leq 4\norm{P}_{\max}^2 \norm{u_1}_1 = 4 \sqrt{n} \norm{P}_{\max}^2 
\quad (\text{since } \Delta \leq \frac{\eta p ||r-\alpha e||_2 \sqrt{n}}{3} \text{ and using H\"older's inequality}). \label{eq:w3_infty_bd}
\end{align}
%
%
Plugging \eqref{eq:linf_w1_bd}, \eqref{eq:w2_infty_bd}, \eqref{eq:w3_infty_bd} in \eqref{eq:u2til_inf_bd_init}, we obtain
%
%
\begin{align*}
\norm{\tilde{u}_2 \mp \det(O) u_2}_{\infty} 
&\leq 4\norm{P}_{\max}\left(2 + \frac{\sqrt{n}(M-\alpha)}{\norm{r-\alpha e}_2} \right) + 4 \sqrt{n} \norm{P}_{\max}^2 \\
&= 4\norm{\Uhat - UO}_{\max}\left(2 + \frac{\sqrt{n}(M-\alpha)}{\norm{r-\alpha e}_2} \right) + 4 \sqrt{n} \norm{\Uhat - UO}_{\max}^2.  
\end{align*}
%
%
The above bound is true for any orthogonal matrix $O$, it is not difficult to see that there exists an 
orthogonal matrix $O = O^*$ such that $\Uhat$ is ``aligned'' with $UO^*$. 
Indeed, for any orthogonal $O$, we first obtain via triangle inequality that 
%
%
\begin{align} \label{eq:linf_temp_4}
  \norm{\Uhat - UO}_2 \leq \norm{(I-UU^T) \Uhat}_2 + \norm{UU^T \Uhat - UO}_2 
	= \norm{\sin \Theta(\calR(U), \calR(\Uhat))}_2 + \norm{U^T \Uhat - O}_2.
\end{align}
%
Denoting $\tilde{U} \tilde{D} \tilde{V}^T$ to be the SVD of $U^T \Uhat$, we 
choose $O = O^* = \tilde{U} \tilde{V}^T$ (so $O^*$ is orthogonal). Denoting $\theta_p$ to be the 
principal angle between $\calR(U), \calR(\Uhat)$, we obtain   
%
\begin{align*}
  \norm{U^T \Uhat - O^*}_2 = \norm{I - \tilde{D}}_2 = 1- \cos \theta_p \leq \sin \theta_p = \norm{\sin \Theta(\calR(U), \calR(\Uhat))}_2.
\end{align*}
%
Plugging this in \eqref{eq:linf_temp_4} leads to 
%
%
\begin{align*}
\norm{\Uhat - UO^*}_2 
&\leq 2 \norm{\sin \Theta(\calR(U), \calR(\Uhat))}_2 \\
&\leq \frac{ 2\Delta }{  \eta p  \sqrt{n} \norm{r-\alpha e}_2 - \Delta } \quad \text{(see proof of Lemma \ref{lem:wedins_bd_ero})} \\
&\leq \frac{3\Delta}{\eta p \sqrt{n} \norm{r-\alpha e}_2}. \quad \text{(since } \Delta \leq \frac{\eta p ||r-\alpha e||_2 \sqrt{n}}{3} \text{)}
\end{align*}
%
\end{proof}
